Potential Gap: Using Reactive Policies to Guarantee Safe Navigation

This paper considers the integration of gap-based local navigation methods with artificial potential field (APF) methods to derive a local planning module for hierarchical navigation systems that has provable collision-free properties. Given that APF theory applies to idealized robot models, the provable properties are lost when applied to more realistic models. We describe a set of algorithm modifications that correct for these errors and enhance robustness to non-ideal models. Central to the construction of the local planner is the use of sensory-derived local free-space models that detect gaps and use them for the synthesis of the APF. Modifications are given for a nonholonomic robot model. Integration of the local planner, called potential gap, into a hierarchical navigation system provides the local goals and trajectories needed for collision-free navigation through unknown environments. Monte Carlo experiments in benchmark worlds confirm the asserted safety and robustness properties by testing under various robot models.

==> figures/hier_structure.tex <==
\tikzstyle{block} = [draw, rectangle, text centered, thick,rounded corners=2pt,
                     minimum height=1.5em, minimum width=5em, inner sep=4pt]
\tikzstyle{typical} = [fill=white!95!black]
\tikzstyle{reddish} = [draw=red,fill=white!95!red]
\tikzstyle{blueish} = [draw=blue,fill=white!95!blue]
\tikzstyle{greenish} = [draw=green!40!gray,fill=white!95!green]
\tikzstyle{longblock} = [draw,rectangle,text centered,thick,rounded corners=2pt,
                     minimum height=1.5em, minimum width=8em, inner sep=4pt]
\tikzstyle{largeBlock} = [draw, rectangle, thick,
                     minimum height=19em, minimum width=35em, inner sep=4pt]
\tikzstyle{smallBlock} = [draw, rectangle, text centered,
                     minimum height=14em, minimum width=22em, inner sep=4pt]
\tikzstyle{dashedBlock} = [draw, dashed, rectangle,
                     minimum height=2em, minimum width=4em, inner sep=4pt]
\tikzstyle{newtip} = [->, very thick]
\tikzstyle{bidir} = [<->, very thick]
\tikzstyle{newtip_dashed} = [->, very thick, dashed]
\begin{tikzpicture}[auto, inner sep=0pt, outer sep=0pt, >=latex]
  % Column 1 - relative to laserscan block and then north.
  \node[block, reddish] (laserscan) {Laserscan};
%  \node[block, typical, anchor=south] (stereo)  
%    at ($(stixel.south) + (0, 1.0)$)  {stereo};
  \node[anchor=south] (goal) at ($(laserscan.north) + (0, 1.0)$) {Goal};
    
  % Column 2
  \node[block,reddish,anchor=west] (egocircle) 
    at ($(laserscan.east) + (1.00, 0)$) 
    {\centering Egocircle};
  \node[block, typical, anchor=south] (costmap)  
    at ($(egocircle.north)+(0, 1)$)
    {\centering World Map};
%  \node[block,reddish,anchor=north,text width=3.5em] (cc)  
%    at ($(egocircle.south) - (0, 0.75)$)   {\centering collision \\ checking};

  % Column 3
  \node[longblock, typical, anchor=west] (global) 
    at ($(costmap.east) + (2.0, 0)$)  
    {\centering Global Planner};
  \node[longblock, blueish, anchor=west, text width=8em] (gap) at (egocircle-|global.west)
    {\centering Gap Generation \\ and Selection};

  \node[longblock,blueish,anchor=north, text width=8em] (traj) 
    at ($(gap.south) - (0, 0.5)$) {\centering Multi-Trajectory \\ Synthesis};
  
  \node[longblock,blueish,anchor=west, text width=8em] (score) 
    at ($(traj.east) + (0.5, 0)$) {\centering Trajectory \\ Scoring};
    
  \node[longblock,blueish,anchor=north, text width=8em] (controller) 
    at ($(score.south) - (0, 0.8)$) {\centering Trajectory \\ Controller};
    
  % Surrounding block for local planner
  \node[smallBlock, draw=blue!70!black,anchor=north] (local) 
    at ($(gap)!0.09!(gap) + (1.8, 1)$){};
  \node[anchor=north] (localtext) at ($(local.north) - (0, 0.05)$ ) 
      {\sc Potential Gap Local Planner};

  % Big surrounding block
  \node[largeBlock, draw=blue!70!black,anchor=north] (planning) 
    at ($(global)!0.09!(costmap) + (0.6, 0.8)$){};
  \node[anchor=north] (planningtext) at ($(planning.north) - (0, 0.05)$ ) 
      {\sc Hierarchical Navigation System};

  % Arrows - standard parts.
%  \draw[newtip] (stereo.south) -- (stixel.north);
  \draw[newtip] (laserscan.east) -- (egocircle.west);
  %\draw[newtip] ($(stixel.east)!0.5!(egocircle.west)$) |- (costmap.west);
  \draw[newtip] (egocircle.north) -- node [midway,right,xshift=2pt]{sensor info} 
    (costmap.south);
  \draw[newtip] (costmap.east) -- (global.west);
  \draw[newtip] (egocircle.east) -- (gap.west);
  \draw[newtip] (gap.south) -- (traj.north);
  \draw[newtip] (traj.east) -- (score.west);
  \draw[newtip] (score.south) -- node [midway,left,xshift=-3pt]{Recent Best Trajectory}(controller.north);
  
  \draw[newtip,<-] (gap.east) -- (gap.east-|score.north) |- node[midway,right,xshift=8pt,yshift=15pt]{Replan}(score.north);

%  % Arrows - new parts.
%  \draw[newtip,<->](cc.east) --node[midway,yshift=2pt]{precheck} (NI.west); 
  \draw[newtip] ($(goal.east)+(3pt,0pt)$) -- (goal.east-|planning.west);
%
%  \draw[newtip] ($(local.south) - (0, 0)$) -- (NI.north);
%  \draw[newtip] (NI.east) -- (following.west);
%
%  \draw[newtip](following.north) -- (replan.south); 
%  \draw[newtip](NI.north east) to[in=250] ([xshift=-5pt]replan.south);
%  \draw[newtip](replan.south west) -- (local.east);
%  \draw[newtip](replan.north west) -- (global.east);

  % Level text.
  \node[anchor=north west, xshift=5pt] (LT) at (planning.north east)
   {\sc Level};
  \node[anchor=center] at (LT|-global) {High};
  \node[anchor=center] at (LT|-local) {Mid};
  \node[anchor=center] at (LT|-controller) {Low};
\end{tikzpicture}
